Curiosity-Driven Testing for Sequential Decision-Making Process

Sequential decision-making processes (SDPs) are fundamental for complex real-world challenges, such as autonomous driving, robotic control, and traffic management. While recent advances in Deep Learning (DL) have led to mature solutions for solving these complex problems, SDMs remain vulnerable to learning unsafe behaviors, posing significant risks in safety-critical applications. However, developing a testing framework for SDMs that can identify a diverse set of crash-triggering scenarios remains an open challenge. To address this, we propose CureFuzz, a novel curiosity-driven black-box fuzz testing approach for SDMs. CureFuzz proposes a curiosity mechanism that allows a fuzzer to effectively explore novel and diverse scenarios, leading to improved detection of crashtriggering scenarios. Additionally, we introduce a multi-objective seed selection technique to balance the exploration of novel scenarios and the generation of crash-triggering scenarios, thereby optimizing the fuzzing process. We evaluate CureFuzz on various SDMs and experimental results demonstrate that CureFuzz outperforms the state-of-the-art method by a substantial margin in the total number of faults and distinct types of crash-triggering scenarios. We also demonstrate that the crash-triggering scenarios found by CureFuzz can repair SDMs, highlighting CureFuzz as a valuable tool for testing SDMs and optimizing their performance.

==> sections/problem.tex <==
\section{Problem Definition}
\label{sec:problem}

\subsection{Assumption}
Two main components in the context of MDP are the agent and the environment. In our scenario, the agent is an AI-powered decision-making entity. The agent would perform a set of actions while interacting with the environment in order to achieve certain goals. The agent would select actions based on its policy, which is learned during the training process. When conducting the fuzzing process, we assume that the policy of the agent is fixed. \toolname conducts the fuzz testing in a black-box manner. In other words, \toolname does not require access to the internal logic of the agent, and we also are not aware of the transition dynamics or the reward mechanism of the environment. However, we are known of the state space of the environment, the action space of the agent, and how to formulate a legitimate space. Given a particular state, we can obtain the corresponding action from the agent. By interacting with the environment, \toolname would get a sequence of state and action pairs. 


\subsection{Testing Oracle}
Our testing oracle is defined in the same way as Pang et al.~\cite{MDPFuzz}. We aim to reveal crashing-triggers states or functional faults, which eventually lead to abnormal termination of the environmental systems (e.g., crashing into pedestrians in the scenario of autonomous driving).

